Message Time of Arrival Codes: A Fundamental Primitive for Secure Distance Measurement

Secure distance measurement and therefore secure Time-of-Arrival (ToA) measurement is critical for applications such as contactless payments, passive-keyless entry and start systems, and navigation systems. This paper initiates the study of Message Time of Arrival Codes (MTACs) and their security. MTACs represent a core primitive in the construction of systems for secure ToA measurement. By surfacing MTACs in this way, we are able for the first time to formally define the security requirements of physical-layer measures that protect ToA measurement systems against attacks. Our viewpoint also enables us to provide a unified presentation of existing MTACs (such as those proposed in distance-bounding protocols and in a secure distance measurement standard) and to propose basic principles for protecting ToA measurement systems against attacks that remain unaddressed by existing mechanisms. We also use our perspective to systematically explore the tradeoffs between security and performance that apply to all signal modulation techniques enabling ToA measurements.

==> analysis_old.tex <==
%!TEX root =  mtac_main.tex
\section{Analysis}

\textcolor{blue}{Here we need to have a simulation-based validation of our model.}

\textcolor{red}{TODO: Why not just cap per-pulse contribution to statistics? However, based on what?}

\textcolor{blue}{Move from check on (easily spoofed) mean to a check of signal variability.}

Goal here is to find different choices of checks that lead to negligible attacker advantages from redundant encodings.

Motivation: Signals need to be 'close' on the pulse level. Receiver needs to aggregate. We want to hide aggregation. Result from random projetions says that $r_{ij} \in \{-1,1\}$ allows to build arbitrary good length estimator. Advantage of 'hidden' length estimator?

Idea for evaluation: Pulse-guessing probability needs to be folded with Q function output in order to arrive at overall attack success probability.

UWB pulse sequence for the transmission of bits. The bits are recovered based on hard decisions applied on orthogonal subsets of this sequence. Theoretical insight is that message time authentication is not directly linked to this decoding, it can be run in addition. It has the nature of a \emph{redundant} check. Permutations for diffusion of individual pulse contributions. Unmatched rx filter for confusion of pulse contribution to statistics. Tradeoff with performance. That's why we separate it from the bits. Bits: Many binary hypothesis tests that need to function robustly. Time authentication: One additional hypothesis test on cryptographically established statistics.


%\subsection{Checks are random projections}
%\textcolor{red}{Irrespective if choice of tests is hidden from attacker or not.}
%
%Sum of projections is an estimator for the length of the received signal. Number of estimators required depends on variance of the estimators!~\cite{database_friendly}. Important insight is that fully randomizing the tests stills allows building an arbitrariy good estimator of overall signal, in the limit for many tests.
%
%Steps:
%\begin{itemize}
%\item Build pulse-level model based on bits and overall receive power.
%\item Obtain expected rx statistics by applying random projections to pulse-level model.
%\item Obtain rx statistics by applying random projections to received pulses.
%\item Take distance between model and rx statistics.
%\item Apply hypothesis test on this distance.
%\end{itemize}
%
%Our assumptions on the receiver requires us to aggregate parts of the signal to statistics, on which we apply tests. \emph{How} we aggregate needs to be hidden from an attacker. Also, minimize feedback about attack progress. This suggest also randomizing the polarity of the projection. In some sense, we apply a generalized (indirect) correlation. Therefore, we have to choose for each check a subset of pulses that are aggregated. In general, we can represent this operation as an inner product
%\[\sigma_i = <s,p_i>.\]
%Statistics $\sigma_i$ can be aggregated as sum or fed directly into a hypothesis test.
%
%\begin{figure}
%	\centering
%	\includegraphics[width=1 \linewidth]{img/rand_proj.pdf}
%	\caption{.}
%	\label{fig:signal}
%\end{figure}
%
%\subsection{Different choices for the set of projections}
%Matched, unmatched. Unmatched binary does have good properties~\cite{}. Matched is more prone to power increase attacks.
%
%\subsection{Bounding the attack success rate}
%If we don't consider noise, we can fully optimize the detecton towards security without performance drawbakcs. This means unmatched projections. For the sum of all statistics, we can everage Johnson-Lindenstrauss (JL)-embeddings. Legitimate and attacker signals are given by points in $\mathbb{R}^n$. $n^{-\beta}$
%\textcolor{red}{TODO: approximate this with first k components, i.e. those that allow for proper hypothesis testing.}
%
%\subsubsection*{Lower bounding the attack distance}
%$\varepsilon$ Depends on the pulse-level distance of alternative hypotheses. Also depends on the decoding applied. What is the distance between signals of two frequencies? Difference of pulse-level contribution to receiver-side statistics under different attacker guesses. What if, say, frequency and phase are changed in ways unforeseen by the attacker?
%%\subsubsection*{We need enough power in the checks}
%%In the worst case, we have to be able to detect $\varepsilon$ fraction of check statistics as legitimate. I.e., the decision threshold needs to be above the sensitivity of the receiver.
%
%\subsubsection*{Probability of distance preservation}
%Here we use existing results for random projections.
%
%\begin{equation}
%\label{eq:jl_bound}
%d \geq \frac{4 + 2\beta}{\varepsilon^2/2 - \varepsilon^3/3}\log(n)
%\end{equation}
%
%\begin{figure}[!t]
%\centering
%\includegraphics[]{plots/num_projections.pdf}
%\caption{Bounds on the probability of attack success vs. the number of checks, for different relative distortions.}
%\label{fig_sim}
%\end{figure}
%
%$d$ is the number of projections, $n$ is the number of guessing attempts, $\varepsilon$ is the relative distortion, $n^{-\beta}$ is the probability.
%
%TODO: Again, here a convolution might be required based on the likelihood of the attacker guessing a certain fraction of pulses and the probability of then detecting the deviation with random projections. This allows to make sense of the results for varying pulse numbers.
%
%\subsubsection*{Transmitting bits}
%Attacker doesn't know the bits. We assume full pulse-level entropy.  Bit transmission essentially necessitates a pre-agreed set of orthogonal checks. Therefore, we do not need to maintain distances between alternative hypotheses with random projections, since we now the dimensions containing the bit information. PR means pulses are reordered. We have different scenarios:
%\begin{itemize}
%    \item If bits won't be checked: Attacker gets the bits wrong or not (PR or not). The bits are then set. Additional checks have to be consistent. Security fully relies on additional checks.
%    \item If PR is used and k out of n bit errors will be detected:
%    \item If PR is used and all bits will be checked: Here, the bits equate to orthogonal additional checks.. TODO: what is the difference of these orthogonal checks and the distribution we rely on for the bound in Equation~\ref{eq:jl_bound}?
%\end{itemize}
%\begin{table}
%    \centering
%    \ra{1.5}
%    \begin{tabular}{llll}
%        \toprule
%         & no bit check & k/n check & full check \\
%         \midrule
%         PR & $P_{win}^{<n_{c}>}$ & ? & $P_{win}^{<n_{c}+n_{b}>}$ (?)  \\
%         no PR & $P_{win}^{<n_{c}>}$ & $P_{win}^{<n_{c}>}$ & $P_{win}^{<n_{c}>}$  \\
%         \bottomrule
%         \vspace{-10pt}
%    \end{tabular}
%    \caption{Bit transmission and security}
%    \label{tab:bit_checks}
%\end{table}
%
%\subsubsection*{Why use more or fewer pulses?}
%Bound on $\varepsilon$ becomes better. More unique projections. Number of pulses needs to exceed sensitivity at least twice.
%
%\subsection{No strategy helps}
%All strategies involve introducing biases. We detect exactly this with random projections. Alternative is pulse-level guessing. Pulse-level guessing doesn't allow to take advantage of quantization effects. The most effective strategy in that sense is easiest detected with additional checks. (The more the attacker optimizes for k checks, the more effective the n-k remaining checks become.)
%
%TODO: Discover the tension between power-increase strategy (if there is no PR) and number of checks required. $\varepsilon$ for different strategies.

\subsection{Fully hidden checks}
Projection matrix $R$, defined as a $n_{P} \times n_{proj}$ random matrix $R\leftarrow\{-1,1\}^{n_{P} \times n_{proj}}$.
%\[r_{i,j} = \begin{cases} +1, \text{with probability }1/2 \\
%-1, \text{with probability }1/2 \end{cases}. \]

Legitimate signal is a random pulse sequence $p_L~\leftarrow~\{-1,1\}^{n_{p}}$.

TODO: Do the statics become optimal (whatever that means) after many projections?
Fully random -> Mean of diff stat increases with number of bits increasing.
Only matched -> Mean saturates and only distribution becomes more focused.

ONe intuition for fully random checks is that they do not test the mean, which can be easily spoofed by the attacker, but the variability across multiple pulses.

Receiver-side statistics
\begin{equation}
\label{eq:random_projection}
S = \frac{1}{k} pR
\end{equation}

Assume pulse sequence is known. Test hypothesis on $S_{diff} = \vert S - \hat S \vert$. For some noise-dependent threshold $T$.
\[\mathcal{H}_0:~~~\text{Legitimate plus noise}\]
\[\mathcal{H}_1:~~~\text{Attack}\]

Attack is a signal variability that cannot be explained by noise only. Noise model is circumvented by basing classification performance on configuration chosen for bit transmission. Essential insight is that checking the mean alone is prone to attacks where an attacker only guesses a subgroup of the pulses correctly but carefully adjusts transmission power.

Decision:
\[S_{diff} \lessgtr T\]

\subsection{Legitimate transmission, noise}
\[p_{Rx} = p_{Tx}* h + n,\]
whereas
\[n \sim \mathcal{N}(0, \sigma^2).\]
Per-pulse, first path, time-discrete version
\[\mathbf{p_{Rx}}[k] = a\cdot p_{Tx}(kT) + n(kT), ~ k\in(0,...,n_p-1)\]
Assume channel stationary over one message, i.e. $a$ const, and delay spread less than $T$.

\subsection{Modelling the distribution of S}
Model distribution of $S_{diff}$ (mean and variance) for different priors, i.e. legitimate, noise, attacker, as a function of noise level and calibration error.


We can upper-bound the variance by considering a Normal approximation of the binomially distributed accumulation of calibration mismatch.

\textcolor{red}{TODO: There should be a common derivation, originating from the identical, canonical start expression.}
Start from gaussian representation of per-projection stats, consider those to be dependent. This means the projection variance cannot be easily derived as sum of (equivalent) per-pulse variances.

Residual variances:
\begin{itemize}
\item Asymptotic behaviour for high number of checks:

\textcolor{red}{TODO: There should be a proper derivation.}
\textcolor{red}{What we have here is a residual mean due to a low sample count. See standard deviation of mean estimate.}

\[\lim_{n_{proj}\rightarrow\infty} \frac{\sigma_{S_{diff}}^2}{n_p} = \frac{\sigma^2 + \vert a-\hat a\vert^2}{\pi n_p}\]

\item Asympototic behaviour for high number of pulses:

\textcolor{red}{TODO: Does the normalization by number of pulses make sense? Somehow like Eb/N0, normalization of SNR.}

\textcolor{red}{TODO: What could be causes for a calibration error other than noise?}

Per-projection gauss variance:
\textcolor{red}{TODO: This is a simplification, in gneral, there are covariances. However, they go away for $n_{check}<<n_{p}$.}

Intuition: 
Statistics of each projection follow a Gaussian distribution. The variance of the per-projection statistics is given by the sum over the variances of the per-pulse contributions, divided by the scaling factor $n_{proj}^2$ that we use in our definition of the projections (Equation~\ref{eq:random_projection}).
\textcolor{red}{TODO: Isn't this the sample variance? In the simulations, yes. But we use a high number of runs there...}

Contribution of each pulse to per-projection stat variance:
\[\sigma_{pp} (per_p, within_{proj}) = \sqrt{\sigma_{n}^2 + \vert a-\hat a\vert^2}\]


Per-pulse contribution to variance of sample mean:
\[\sigma_{\mu} (per_p, within_{proj}) = \frac{\sqrt{\sigma^2 + \vert a-\hat a\vert^2}}{\sqrt{n_p}\cdot n_{proj}}\]

Variance of sample variance:
\[\hat{\sigma}_{pp} = \frac{\sqrt{2}}{\sqrt{n_p - 1}}\cdot \sigma_{pp}^2\]
We define $\sigma_g$ to be the variance of the inner product per projection, before taking the absolute value. Factor $n_{proj}$ comes in due to our normalization chosen in application of random projection.

\textcolor{red}{TODO: Check normal model for binomial}

\textcolor{red}{TODO: Write down $\sigma_g$ as mean and some variation term.}

Finding from simulation: For increasing numbers of projections, the distribution of $\vert\sigma_g\vert$ will more and more resemble a gaussian.


This we were able to validate by simulation:
\[\sigma_g(per_{proj}, within_{rep}) \sim \left( \frac{\sqrt{n_p\cdot\sigma_{pp}^2}}{n_{proj}},  \hat{\sigma}_{pp}^2 \right)\]
\[\sigma_g = \sqrt{n_p + \frac{2}{n_p - 1}\cdot \sigma_{pp}^2}\cdot \sigma_{pp}\]
\[\mu_{folded} = \sigma_g\sqrt{\frac{2}{\pi}}\]

\textcolor{red}{The quality of the variance estimate of projections is limited by the number of pulses. Random projections is application of inner product with zero-mean mask (at high number of proj) on limited number of pulses, that might have a mean sampling error. Due to $n_{proj}$ high and mask zero mean, the projection stats (before abs) are also zero-mean. However, the variance is increased due to the mean sampling error. TODO: How much is the variance per proj increased?}


\textcolor{red}{This is a simplification step. In general, the statistics of different projections are correlated - becaus the per-pulse sample.}
\textcolor{red}{Maybe covariance comes in only in regime for very low number of pulses, i.e. when we get close to exhausting the space of projections. Conclusion: focus on effect of sample mean of pulse polarities on variance of stats.}

We use the expression of the variance for the folded normal distribution. Under the hypothesis that $g$ is Gaussian.
\textcolor{red}{TODO: check behaviour of $\frac{\mu_g}{\sigma_g}$}
\[\mu_{\vert g\vert} = \sigma_g\sqrt{\frac{2}{\pi}}e^{(-\mu_g^2/2\sigma_g^2)} + \mu_g\left(1-2\Phi\left(\frac{-\mu_g}{\sigma_g}\right)\right)\]
\[\sigma_{\vert g\vert}^2 = \mu_g^2 + \sigma_g^2 - \mu_{\vert g\vert}^2\]

\[\sigma_{S_{diff}}^2 = n_{proj}\cdot \sigma_{\vert g\vert}^2\]
%\[\sigma_{S_{diff}}^2 = \sigma_{abs}^2 + \]

$\rho$ denotes the average correlation of distinct projections.

%\[\hat{\operatorname{Cov}} = \sigma_{abs}^2 + n_{proj}\cdot \rho\]


In simulations, this model is only accurate for high numbers of projections.
\[\sigma_{S_{diff}}^2 = n_{proj}\cdot\sigma_g^2\cdot \left(1 - \frac{2}{\pi}\right)\]
\textcolor{red}{TODO: }
\[\frac{\sigma_{S_{diff}}^2}{n_p} = \left(1 - \frac{2}{\pi}\right) \cdot \left[ \frac{\sigma^2 + \vert a-\hat a\vert^2}{n_{proj}}  + \frac{\sigma^2 + \vert a-\hat a\vert^2}{n_p\cdot n_{proj}}\right]\]
\[\lim_{n_{p}\rightarrow\infty}  \frac{\sigma_{S_{diff}}^2}{n_p} = \left(1 - \frac{2}{\pi}\right)  \frac{\sigma^2 + \vert a-\hat a\vert^2}{n_{proj}}\]
\end{itemize}

\subsection{Conclusion}
Insights from random projections:
\begin{itemize}
\item As the number of random checks is increased, the probability of winning decreases exponentially.
\item We can achieve security for any strategy by adding tests. Limitation: Channel- and noise-free environment.
\end{itemize}

Insights from simulations:
\begin{itemize}
\item Noise causes false positives. In order to place the decision boundary meaningfully we either rely on a subset of random projections that is partially algined with the legitimate sequence (and zero-thr) or use a power estimate.
\item If we don't have a model for the expected power per symbol, we can focus on a subset of the tests. I.e., check if tests that end up in statistics significantly removed from zeros have the correct sign. However, this way, we do not sample the tests truly randomly anymore, as tests that are close to the legitimate signal are preferred.
\item Signal level at legitimate symbols could be considered a power-level \emph{commitment}. Checks are redundant anyway. Power measured in bit reception could inform the tests under the hypothesis that it is evenly spread out over the pulses (how it should be). Checks are then about checking for the contrary.
\item We don't need to explore attack strategies. We can, however, test our checks by providing part of the legitimate pulse sequence to the attacker. If it is optimal under this model for the attacker not to amplify the known signal part, our hypothesis is confirmed.
\item More noise in the legitimate signal has no effect on negatives, only false positives go up. It is therefore possible to make a good choice of the number of tests, given a certain number of bits. FPR performance then depends on noise.
\item \textcolor{red}{What is the impact on security if TOPK is used instead of SUM?} Performance seems to be more stable. However, we reduce the capability of distinguishing fake-high from low. Stats/distance required for both distinguishing signal from noise and validate signal. Approach: Simulate 'good' attacks.
\item Attacker noise helps the detection of attacks.
\end{itemize}

Attacker has to commit to an encoding which is hidden to the receiver (less resolution). Commitment is revealed by additional checks. What about UWB-PR? Commitment is revealed by checking the bits, which are given. By sending a certain bit sequence, the attacker commits to having knowledge about the underlying modulation.

%\begin{figure}[t]
%	\begin{center}
%%		\includegraphics[scale=1]{plots/jl_sim_s_diff_sum.pdf}
%		\caption{Attack statistics (solid) as well as noise-induced statistics (dashed). Gap widens for more checks as well as more bits, which means fewer classification errors. For any noise profile, we find a number of checks and bits, such that EER goes to zero (?). TODO: given a number of bits, what's the limit in number of checks that help, i.e., marginal effect of more checks? Might be related to CDMA theory.}
%	\end{center}
%\end{figure}
%
%\begin{figure*}[t]
%	\begin{center}
%%		\includegraphics[scale=1]{plots/jl_sim_pwin.pdf}
%%		\includegraphics[scale=1]{plots/jl_sim_fpr.pdf}
%		\caption{Probability of winning (left) and false positive rate (right) as a function of the number of checks for different numbers of bits. Each bits consists of 16 pulses. More checks strictly improve the classification performance, as both $P_{win}$ and the FPR get smaller.}
%		\label{fig:decrease_combined}
%	\end{center}
%\end{figure*}


\section{Simulation Results}
We consider on over-approximation of a distance-reducing guessing attacker. The attacker's goal is to guess elements of binary pulse sequence in advance in order to manipulate the time-of-flight measurement at the receiver. An attacker generally uses the fact that the mean of a set of pulses is information-bearing. Adaptive increases of power can help such an attacker to compensate for wrong guesses.

\begin{figure}[]
	\begin{center}
		\includegraphics[scale=1]{plots/p_att_ex.pdf}
		\caption{Example legitimate and attack sequence}
	\end{center}
\end{figure}

\begin{figure*}[t]
	\begin{center}
		\includegraphics[scale=1]{plots/jl_sim_s_diff_sum_rd_orthom.pdf}
		\includegraphics[scale=1]{plots/jl_sim_s_diff_sum_rd_full.pdf}
		\caption{Difference of statistics under attack and legitimate transmission, together with an equal-FPR decision threshold. We see that the gap widens for more bits, leading to a lasting exponential decay in $P_{win}$.}
		\label{fig:jl_sim_diff}
	\end{center}
\end{figure*}

\begin{figure*}[t]
	\begin{center}
		\includegraphics[scale=1]{plots/jl_sim_pwin_orthom.pdf}
		\includegraphics[scale=1]{plots/jl_sim_pwin_full.pdf}
		\caption{Probability of winning for 128 matched (left) and unmatched (right) tests under an SNR of 0dB as a function of the number of bits per frame. Decision threshold is chosen such that the resulting FPR matches the baseline scenario of 16 pulses per bit. Matching the tests to the expected sequence is associated with a better concrete security level. However, in the limit for many proujections, even fully unmatched projections can satisfy the MTAC security goal.}
		\label{fig:jl_sim_pwin}
	\end{center}
\end{figure*}



==> discussion.tex <==
%!TEX root =  mtac_main.tex
\section{Lessons Learned}
\label{sec:discussion}


%\subsection{Related schemes}
%
%\subsubsection*{Correlation sequence}
%A standard way of signal time acquisition is correlating an incoming signal with the expected signal shape and locking to the peak. One could argue that secure ToA verification could be achieved by checking for this peak. However, we know that tests for time acquisition and content verification should not be coupled~\cite{poturalski2010cicada}. If only used for content verification, the security of such an approach, however, depends on the detailed test the receiver applies, i.e., the degree to which the relative quality of the peak (peak-to-average ratio) is considered. The power level at the peak itself can easily be steered to a desired value by an attacker relying on a power-increase strategy. Therefore, tests based on a) the existence of a correlation peak or b) the peak power level alone are both not secure.
%
%However, we argue that, if employed correctly, a correlation could theoretically be used for content verification. The side peaks of the correlation sequence are essentially the integration of the incoming signal after a random polarity switch, as the time-shifted version of the expected signal does not match the received signal. The energy of the side peaks can be considered an estimator for the underlying signal variance. Testing the peak-to-average ratio of a correlation sequence could, therefore, potentially be a secure approach for ToA-verification. This because an attacker will increase the variance through guessing errors and a potential power-increase strategy. However, due to the side-peaks being non-zero even in a benign scenario there would likely be an increased tendency for false positives compared to our approach.
%
%\subsubsection*{Hidden encoding: UWB-PR}
%Secure ToA-verification based on the bit-level content can to some extent be achieved by hiding the mapping from pulses to bits as in~\cite{singhuwb}. The drawback of this scheme is that it incentivizes the attacker to transmit a small number of strong pulses, and, in case their polarity is correct, hope that they align with the bits. This method, therefore, has a relatively coarse quantization loss that can be exploited by an attacker. While such a scheme does not require a decision threshold for attack detection, it also does not allow for tuning the security level and bit-wise performance independently. In general, this leads to lower security guarantees compared to our proposal.


%\subsection{Lessons Learned}
%What did the community miss?
Since our proposal provides a fundamentally secure physical-layer building block for ToA measurement, this changes prevailing assumptions on the design of higher level protocols. In~\cite{clulow2006so}, Clulow et al. put forward principles for distance bounding:
\blockquote{"We propose a number of principles to adhere to when implementing distance-bounding systems. These restrict the choice of the communication medium to speed-of-light channels, the communication format to single bit exchanges for timing, symbol length to narrow (ultra wideband) pulses, and protocols to error-tolerant versions. These restrictions increase the technical challenge of implementing secure distance bounding."}

Given the above designs, these recommendations don't seem to hold up. 
Also, the recommendation to single bit timing is not only not needed but also are fairly wasteful.  Again, from~\cite{clulow2006so}:

\blockquote{"We show that proposed distance-bounding protocols of Hu, Perrig, and Johnson (2003), Sastry, Shankar and Wagner (2003), and {\v{C}}apkun and Hubaux (2005, 2006) are vulnerable to a guessing attack where the malicious prover preemptively transmits guessed values for a number of response bits."}

In this work, we show that these vulnerabilities are an artifact of a somewhat naively designed physical layer and modulation, and can be addressed purely on the physical layer. The problem and its solution are orthogonal to the design and security of the protocol that builds in it, which operates on a different level of abstraction, making different assumptions about the security parameter (i.e., the bits) making up the nonces. These protocols not addressing the physical layer does not mean they are necessarily vulnerable. If coupled with a physical layer that is in line with our design, they are secure, within the performance region we point out.
%These are not really correct since such protocols didn't specify the physical layer. Exchange of entire nonces is, in fact, secure and the attacks, therefore, don't hold. 

%Error-tolerance? Not clear, this can be achieved at the physical layer. Don'add error tolerance to the encoding used for secure distance measurement. Verification of the bit-level information can also be achieved by sending a MAC separately, over an arbitrary channel, without ToA guarantees.


%\subsection{Limitation: Untrusted Prover}
%To extend the scheme to an untrusted prover, one has to tie the timed response to challenge content that is itself timed. This necessitates a prover radio that can intermingle incoming pulse-level random sequence with its nonce,  while itself unable to detect the challenge content.
%With an untrusted prover, we cannot rely on any information quantization (i.e., aggregation) in the challenge-response phase of the protocol. Instead, a prover needs to modulate secret information directly on the incoming pulse sequence. Under the assumption that such a radio device exists, our components, i.e., a hidden XOR-sequence as well as a distortion test can secure ranging against an untrusted prover.



==> temp <==
% Mtac name, #1: MTAC type (e.g., A)
\newcommand{\mtac}[1]{\mathit{MTAC-#1}}

% Forge experiment, #1 MTAC type (e.g., A), #2: Set of algorithms (e.g., \Pi), #3: Forger (e.g., A(\alpha))
\newcommand{\mtacforge}[3]{\cmathit{Mtac_{#1}-forge}(#2,#3)}

% Forge experiment, #1: MTAC type (e.g., A), #2: Forger (e.g., A(\alpha)), #3: Advancment goal (e.g., \delta), #4: Set of algorithms (e.g., \Pi), #5: Security parameter (e.g., n_p)
\newcommand{\mtacforgealt}[5]{\mathit{Mtac_{#1}-forge}_{#2,#3,#4}(#5)}

% Forger advantage, #1: MTAC (e.g, MTAC-A), #2: Set of algorithms (e.g., \Pi), #3: Forger (e.g., A(\alpha))
\newcommand{\mtacadv}[3]{\mathit{Adv}^{#1}_{#2}(#3)}

% Max forger advantage (insecurity function), #1: MTAC (e.g., MTAC-A), #2: Set of algorithms (e.g., \Pi) 
\newcommand{\mtacadvmax}[2]{\textbf{Adv}^{#1}_{#2}(q,t)}

% Forger
\newcommand{\frgr}{A}

% Forger with arg, #1: Observation delay (e.g., \alpha)
\newcommand{\frgarg}[1]{\frgr(#1)}

% Set of algorithms
\newcommand{\algset}{\Pi}

% Generation algorithm
\newcommand{\genalg}{\mathit{Gen}}

% Mtac algorithm
\newcommand{\mtacalg}{\mathit{Mtac}}

% Verification algorithm
\newcommand{\vrfyalg}{\mathit{Vrfy}}

% Advancement mode ID
\newcommand{\advid}{A}

% Delay mode ID
\newcommand{\delid}{D}

% Observation delay
\newcommand{\obsdel}{\alpha}

% Advancement goal
\newcommand{\advgoal}{\delta}

